High energy bounds on wave operators

The wave operators $W_\pm(H_1,H_0)$ of two selfadjoint operators $H_0$ and $H_1$ are analyzed at asymptotic spectral values. Sufficient conditions for $\|(W_\pm(H_1,H_0)-P_{1}^\mathrm{ac}P_{0}^\mathrm{ac})f(H_0)\| <\infty$ are given, where $P_{j}^\mathrm{ac}$ projects onto the subspace of absolutely continuous spectrum of $H_j$ and $f$ is an unbounded function ($f$-boundedness), both in the case of trace-class perturbations and in terms of the high-energy behaviour of the boundary values of the resolvent of $H_0$ (smooth method). Examples include $f$-boundedness for the perturbed polyharmonic operator and for Schr\"odinger operators with matrix-valued potentials. We discuss an application to the problem of quantum backflow.

==> macros.tex <==
% Layout definitions

\RequirePackage{color}

% \newcommand{\hidetodos}{\renewcommand{\todo}{} \renewcommand{\todonote}{} }
% \newcounter{todo}
% 
% % TODOs
% %\definecolor{todocol}{blue}{0.3}
% 
% \newcommand{\todobox}[1]{
%   \textcolor{blue}{
%     \fbox{\parbox{0.9\textwidth}{#1}}%
%   }
% }
% 
% \newcommand{\todo}[1]{
%   \stepcounter{todo}%
%   \todobox{TODO \arabic{todo}: #1}
% }
% 
% \newcommand{\todonotetag}{TODO\thetodo}
% \newcommand{\todonote}[1]{%
% \stepcounter{todo}%
% {\let\thefootnote\todonotetag
% \footnote{\todobox{#1}}%
% }
% }

% Makrodefinitionen (global)


\def \cbb{\mathbb{C}}
\def \ibb{\mathbb{I}}
\def \nbb{\mathbb{N}}
\def \rbb{\mathbb{R}}
\def \qbb{\mathbb{Q}}
\def \zbb{\mathbb{Z}}

\def \acal {\mathcal{A}}
\def \bcal {\mathcal{B}}
\def \ccal {\mathcal{C}}
\def \dcal {\mathcal{D}}
\def \ecal {\mathcal{E}}
\def \fcal {\mathcal{F}}
\def \gcal {\mathcal{G}}
\def \hcal {\mathcal{H}}
\def \ical {\mathcal{I}}
\def \jcal {\mathcal{J}}
\def \kcal {\mathcal{K}}
\def \lcal {\mathcal{L}}
\def \mcal {\mathcal{M}}
\def \ncal {\mathcal{N}}
\def \ocal {\mathcal{O}}
\def \pcal {\mathcal{P}}
\def \qcal {\mathcal{Q}}
\def \rcal {\mathcal{R}}
\def \scal {\mathcal{S}}
\def \tcal {\mathcal{T}}
\def \ucal {\mathcal{U}}
\def \vcal {\mathcal{V}}
\def \wcal {\mathcal{W}}
\def \xcal {\mathcal{X}}
\def \ycal {\mathcal{Y}}
\def \zcal {\mathcal{Z}}

\def \afk  {\mathfrak{A}}
\def \bfk  {\mathfrak{B}}
\def \dfk  {\mathfrak{D}}
\def \ffk  {\mathfrak{F}}
\def \lfk  {\mathfrak{L}}
\def \mfk  {\mathfrak{M}}
\def \nfk  {\mathfrak{N}}
\def \pfk  {\mathfrak{P}}
\def \vfk  {\mathfrak{V}}
\def \wfk  {\mathfrak{W}}
\def \zfk  {\mathfrak{Z}}

\newcommand{\betav}{\boldsymbol{\beta}}
\newcommand{\thetav}{\boldsymbol{\theta}}
\newcommand{\etav}{\boldsymbol{\eta}}
\newcommand{\lambdav}{\boldsymbol{\lambda}}
\newcommand{\nuv}{\boldsymbol{\nu}}
\newcommand{\zetav}{\boldsymbol{\zeta}}
\newcommand{\piv}{\boldsymbol{\pi}}
\newcommand{\xiv}{\boldsymbol{\xi}}
\newcommand{\varphiv}{\boldsymbol{\varphi}}

\newcommand{\av}{\boldsymbol{a}}
\newcommand{\bv}{\boldsymbol{b}}
\newcommand{\cv}{\boldsymbol{c}}
\newcommand{\ev}{\boldsymbol{e}}
\newcommand{\jv}{\boldsymbol{j}}
\newcommand{\nv}{\boldsymbol{n}}
\newcommand{\pv}{\boldsymbol{p}}
\newcommand{\qv}{\boldsymbol{q}}
\newcommand{\xv}{\boldsymbol{x}}
\newcommand{\yv}{\boldsymbol{y}}
\newcommand{\zv}{\boldsymbol{z}}
\newcommand{\zerov}{\boldsymbol{0}}

% Spacing

\newcommand{\cdotarg}{ \, \cdot \, }

% Operators

\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\re}{Re}

\DeclareMathOperator{\trace}{tr}

\newcommand{\id}{\operatorname{id}}
\newcommand{\idop}{\boldsymbol{1}}
%\def \idop {\mathbb{1}}

\newcommand*\laplace{\mathop{}\!\mathbin\bigtriangleup}

\def \csq {\quad \Rightarrow \quad}

\def \into {\rightarrow}
\def \st {^\ast}
\def \isom {\cong}
\def \restrict {\lceil}

\DeclareMathOperator{\supp}{supp}

\newcommand{\vn}[1]{^{(\smash{#1})}}

% lhs/rhs of equations
\newcommand{\lhs}[1]{\mathrm{l.h.s.}(\ref{#1})}
\newcommand{\rhs}[1]{\mathrm{r.h.s.}\eqref{#1}}

\def \noqed{ \renewcommand{\qed}{} }


\newcommand{\etskp}[2]{\langle #1 | #2 \rangle }

%%% Operator spaces and vector spaces

% Hilbert space (Fock space)
\newcommand{\Hil}{\mathcal{H}}

% Space of vectors of finite particle number
\newcommand{\fpn}{\Hil^{\mathrm{f}}}
\newcommand{\fpno}{\Hil^{\omega,\mathrm{f}}}
\newcommand{\fpnp}{P^\mathrm{f}}


% Bounded operators on H
\newcommand{\boundedops}{\bfk(\Hil)}
\newcommand{\bops}{\bfk}

% Quadratic forms
\newcommand{\qf}{\mathcal{Q}}

% (Local) algebra in general
\newcommand{\A}{\mathcal{A}}
% Standard wedge algebra
\newcommand{\M}{\mathcal{M}}

% Hilbert space (Fock space) scalar product - three different sizes
\newcommand{\hscalar}[2]{\langle #1 , #2 \rangle }
\newcommand{\bighscalar}[2]{\big\langle  #1 , #2 \big\rangle }
\newcommand{\Bighscalar}[2]{\Big\langle  #1 , #2 \Big\rangle }

\newcommand{\expectation}[2]{\langle #1 \rangle_{#2} }


% Norms for quadratic forms
\newcommand{\qfnorm}[2]{\lVert #1 \rVert_{#2}}

% Generic norm
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\bignorm}[1]{\big\lVert #1 \big\rVert}
\newcommand{\Bignorm}[1]{\Big\lVert #1 \Big\rVert}
% Generic norm with subscript
\newcommand{\gnorm}[2]{\lVert #1 \rVert_{#2}}
\newcommand{\biggnorm}[2]{\big\lVert #1 \big\rVert_{#2}}
\newcommand{\Biggnorm}[2]{\Big\lVert #1 \Big\rVert_{#2}}
% Omega norm with subscript
\newcommand{\onorm}[2]{\lVert #1 \rVert_{#2}^\omega}
\newcommand{\bigonorm}[2]{\big\lVert #1 \big\rVert_{#2}^\omega}
\newcommand{\Bigonorm}[2]{\Big\lVert #1 \Big\rVert_{#2}^\omega}

%%% Geometrical regions

\newcommand{\leftwedge}{\mathcal{W}'}
\newcommand{\rightwedge}{\mathcal{W}}

%%% Miscellaneuous symbols

% a,z dagger
\newcommand{\ad}{a^\dagger}
\newcommand{\zd}{z^\dagger}

% left and right ``vector'' distributions
\newcommand{\lvector}[2]{\boldsymbol{\ell}_{#1}(#2)}
\newcommand{\rvector}[2]{\boldsymbol{r}_{#1}(#2)}

% contracted matrix element
\newcommand{\cmeA}[2]{f_{#1}^{\lbrack #2 \rbrack}}
\newcommand{\cmeB}[2]{f_{#1}{\lbrack #2 \rbrack}}
\newcommand{\cme}[2]{\mathchoice{\cmeA{#1}{#2}}{\cmeB{#1}{#2}}{\cmeB{#1}{#2}}{\cmeB{#1}{#2}}}
\newcommand{\cmelong}[2]{f_{#1} \left\lbrack #2 \right\rbrack}

% analytic indicatrix
\newcommand{\oa}{\varpi}

% strip in the complex plane
\DeclareMathOperator{\strip}{S}

% ``affiliated with'' relation
\newcommand{\affiliated}{\mathrel{\eta}}

% tube over a set
\newcommand{\tube}{\mathcal{T}}

% Symmetric group; Sign of a permutation
\newcommand{\perms}[1]{\mathfrak{S}_{#1}}
\DeclareMathOperator{\sign}{sign}

% residue
\DeclareMathOperator*{\res}{res}

% domain
\DeclareMathOperator*{\dom}{dom}

% convex hull and variants
\DeclareMathOperator{\ch}{ch}
\DeclareMathOperator{\cch}{cch}
\DeclareMathOperator{\ich}{ich}
\DeclareMathOperator{\ach}{ach}

% identity (added CJF 7/12/12)
\newcommand{\II}{{\boldsymbol{1}}}

% smooth compactly supported functions (added CJF 7/12/12)
\newcommand{\CoinX}[1]{C_0^\infty({#1})}

% miscellaneous symbols (added CJF 11/2/13)
\newcommand{\LL}{\mathscr{L}}
\newcommand{\xx}{{\sf x}}
\newcommand{\kk}{{\sf k}}


%scattering symbols
\newcommand{\scin}{_\mathrm{in}}
\newcommand{\scout}{_\mathrm{out}}
\newcommand{\Om}{\Omega}

\newcommand{\xfact}{\langle x \rangle}

% fibre hilbert space
\newcommand{\hilf}{\mathfrak{h}}

% Auxiliary Banach space in the smooth method
\newcommand{\Ban}{\mathcal{X}}
\newcommand{\Band}{\mathcal{X}^\ast}
\newcommand{\Banalt}{\mathcal{E}}
\newcommand{\Ah}{\mathcal{B}}
\newcommand{\Ahd}{\mathcal{B}^\ast}

% Projector onto absolute continous spectrum
\newcommand{\pac}[1]{P_{#1}^\mathrm{ac}}

% Moeller operator in/out
\newcommand{\mo}{W}
\newcommand{\mopm}{W_\pm}
\newcommand{\moller}{wave}

% ``almost absolutely continous'' operators
\DeclareMathOperator{\aac}{AAC}

% Gandalf's macros
\newcommand{\Rl}{\mathbb{R}}
\newcommand{\Nl}{\mathbb{N}}
\newcommand{\Ss}{\mathscr{S}}   % Schwartz space
\newcommand{\gti}{\tilde{g}}
\newcommand{\La}{\Lambda}
\newcommand{\Cl}{\mathbb{C}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Hinn}{H_{\rm inner}}
\newcommand{\ot}{\otimes}
\newcommand{\eps}{\varepsilon}
%\newcommand{\dom}{{\rm dom}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\hti}{\tilde{h}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\dr}{{\rm d}}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\slim}{s-lim}
\DeclareMathOperator*{\wlim}{w-lim}

